Efficient Neural Network Analysis with Sum-of-Infeasibilities

Inspired by sum-of-infeasibilities methods in convex optimization, we propose a novel procedure for analyzing verification queries on neural networks with piecewise-linear activation functions. Given a convex relaxation which over-approximates the non-convex activation functions, we encode the violations of activation functions as a cost function and optimize it with respect to the convex relaxation. The cost function, referred to as the Sum-of-Infeasibilities (SoI), is designed so that its minimum is zero and achieved only if all the activation functions are satisfied. We propose a stochastic procedure, DeepSoI, to efficiently minimize the SoI. An extension to a canonical case-analysis-based complete search procedure can be achieved by replacing the convex procedure executed at each search state with DeepSoI. Extending the complete search with DeepSoI achieves multiple simultaneous goals: 1) it guides the search towards a counter-example; 2) it enables more informed branching decisions; and 3) it creates additional opportunities for bound derivation. An extensive evaluation across different benchmarks and solvers demonstrates the benefit of the proposed techniques. In particular, we demonstrate that SoI significantly improves the performance of an existing complete search procedure. Moreover, the SoI-based implementation outperforms other state-of-the-art complete verifiers. We also show that our technique can efficiently improve upon the perturbation bound derived by a recent adversarial attack algorithm.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In Section 5.3, we discuss the complementary nature of the
      proposed techniques with the existing techniques.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{The entire motivation for the research area of neural network verification is to limit potential negative impacts of machine learning systems.  Thus, we believe the appropriate way to contextualize this work is to mention these risks (as we do in the introduction) and offer work like ours as a contribution to the mitigation of such risks.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section 3.1.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Section 3.1.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We have these materials ready, but to anonymize our work, we will wait to release them until the anonymous review period is over.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{ap:details}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See section 5.2.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited all the benchmarks and baselines we evaluated.}
  \item Did you mention the license of the assets?
    \answerYes{See Appendix~\ref{ap:details}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We will release the concrete benchmark sets and the tool once
    the anonymous review period is over.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> pgprimer.tex <==
% Credits: Riad
\ifx\noeditingmarks\undefined
\subsection*{Peanut gallery primer (deleteme)}

\texttt{peanutgallery.sty} provides some commenting and editing functionality.

\texttt{\textbackslash cb},
\texttt{\textbackslash az}, \texttt{\textbackslash gk}, and
\texttt{\textbackslash hw} insert color-coded inline comments.
%
\hw{For example, it looks like this when I comment.}
\az{Test 1.}
\gk{Test 2.}
\cb{Test 3.}

\texttt{\textbackslash CB},
\texttt{\textbackslash AZ}, \texttt{\textbackslash GK}, and
\texttt{\textbackslash HW} insert a tiny vertical bar
\AZ{like this!}
%
and a corresponding margin comment.
%
It's safe to insert a margin comment on a new line, because the command
    includes an \texttt{\textbackslash unskip} that kills prior spacing.
%
\HW{I promise, that's what you want!}
\AZ{test 1}
\GK{test 2}
\CB{test 3}

The \texttt{\textbackslash changebars\{new\}\{old\}} command lets you
    \changebars{show your edits in an explicit way}{change your mind}, which I
\HW{(me)}
frequently find useful.

Finally, if you add \texttt{\textbackslash def\textbackslash noeditingmarks\{\}}
    before \texttt{peanutgallery.sty} gets invoked in \texttt{main.tex},
\GK{it's probably already there and commented out}
then all markings get turned off and the
\texttt{\textbackslash changebars} command does the sensible thing (try it!).

\fi


==> plots/Makefile <==
default:
	Rscript pair-scatter.R
	python get_scatter_pair.py raw_results/Portfolio::Wed_Mar_17_19\:10\:19_2021_-0700::f29c48fac391e73520ff23b5c36bbdff62121324::--sc-pol+--polarity::3600 raw_results/ERAN::Wed_Feb_17_13\:58\:32_2021_-0800::0be1a470a8439cde16950a7dddf7533d99ec6192::--domain\=deeppoly+--numproc\=2::3600 SOI_portfolio ERAN1 pair-scatter-main.csv
	Rscript pair-scatter-main.R -f pair-scatter-main.csv -x SOI_portfolio -y ERAN1 -o pair-scatter-main.png
	python get_main_table.py result_breakdown.csv > main_table.csv

all:
	./get_breakdown.sh > result_breakdown.csv
	./get_breakdown_appendix.sh > result_breakdown_appendix.csv

appendix:
	python get_scatter_pair_appendix.py raw_results_appendix/Portfolio::Wed_Mar_17_19:10:19_2021_-0700::f29c48fac391e73520ff23b5c36bbdff62121324::--sc-pol+--polarity::3600 raw_results_appendix/ERAN%%Wed_Feb_17_13:58:32_2021_-0800%%0be1a470a8439cde16950a7dddf7533d99ec6192%%--domain=deeppoly+--numproc=2%%3600 SOI_portfolio ERAN1 pair-scatter-main-appendix.csv
	Rscript pair-scatter-main.R -f pair-scatter-main-appendix.csv -x SOI_portfolio -y ERAN1 -o pair-scatter-main-appendix.png
	python get_main_table.py result_breakdown_appendix.csv > main_table_appendix.csv



clean:
	rm -f *.png
	rm pair-scatter-main.csv
	rm result_breakdown.csv


==> plots/neural_network.tex <==

\def\layersep{1.5cm}

\begin{wrapfigure}{r}{0.46\linewidth}
  \vspace{-0.5cm}
  \centering
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
  \tikzstyle{every pin edge}=[<-,shorten <=1pt]
  \tikzstyle{neuron}=[circle,fill=black!25,minimum size=13pt,inner sep=0pt]
  \tikzstyle{input neuron}=[neuron];
  \tikzstyle{output neuron}=[neuron];
  \tikzstyle{hidden neuron}=[neuron];
  \tikzstyle{annot} = [text width=4em, text centered]

  % Draw the input layer nodes
  \foreach \name / \y in {1,...,2}
  % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
  \node[input neuron] (I-\name) at (0,-\y cm) {};

  % Draw the hidden layer nodes
  \foreach \name / \y in {1,...,2}
  \node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};

  \foreach \name / \y in {1,...,2}
  \node[hidden neuron] (H2-\name) at (2*\layersep,-\y cm) {};

  % Draw the output layer node
  \foreach \name / \y in {1,...,2}
    \node[output neuron] (O-\name) at (3*\layersep,-\y cm) {};

  % Connect every node in the input layer with every node in the
  % hidden layer.
  \foreach \source in {1,...,2}
  \foreach \dest in {1,...,2}
  \draw (I-\source) edge (H1-\dest) node[right] {\scriptsize 1};

  \foreach \source in {1,...,2}
  \draw (H1-\source) edge (H2-\source);

  % Connect every node in the hidden layer with the output layer
  \foreach \source in {1,...,2}
  \foreach \dest in {1,...,2}
  \path (H2-\source) edge (O-\dest);

  % Annotate the layers
  \node[annot,above of=I-1, node distance=0.4cm] {\scriptsize[-1, 1]};
  \node[annot,above of=I-2, node distance=0.4cm] {\scriptsize[-1, 1]};
  \node[annot,above of=H1-1, node distance=0.4cm] {\scriptsize[-1, 1]};
  \node[annot,above of=H1-2, node distance=0.4cm] {\scriptsize[-1, 1]};
  \node[annot,above of=H2-1, node distance=0.4cm] {\scriptsize[0, 1]};
  \node[annot,above of=H2-2, node distance=0.4cm] {\scriptsize[0, 1]};
  \node[annot,above of=O-1, node distance=0.4cm] {\scriptsize[0, 2]};
  \node[annot,above of=O-2, node distance=0.4cm] {\scriptsize[0, 3]};


  \end{tikzpicture}
\end{wrapfigure}


==> plots/vio-relu.tex <==
\begin{wrapfigure}{r}{0.46\linewidth}
  \vspace{-0.5cm}
  \centering
  \begin{tikzpicture}
    \draw[->, very thick] (-3, 0) -- (3, 0) node[right] {$n^b$};
    \draw[->, very thick] (0, 0) -- (0, 3) node[above] {$n^f$};
    \draw[domain=-2.5:0, very thick, variable=\x, blue] plot ({\x}, {0});
    \draw[domain=0:2.5, very thick, variable=\x, blue] plot ({\x}, {\x});
    \draw[domain=-2.5:2.5, very thick, dashed, variable=\x, blue] plot ({\x}, {0.5*\x+1.25});

    \draw[domain=0:2.5, thick, dashed, variable=\y] plot ({2.5}, {\y});

    \path[fill=red, opacity=0.25] (-2.5,0) -- (0,0) -- (2.5,2.5) -- cycle;

    % annotating l and u
    \node at (0, -0.3) {0};
    \node at (2.5, -0.3) {$u$};
    \node at (-2.5, -0.3) {$l$};

    %points
    \draw[fill=red] (-1.2,0.45) circle (.05);
    \node at (-0.6, 0.45) {\scriptsize $(n^b_0, n^f_0)$};
    \draw[->, densely dotted, thick] (-1.2, 0.4) -- (-1.5, 0.15);
    \draw[->, densely dotted, thick] (-1.2, 0.4) -- (-1.2, 0.05);
    \draw[->, densely dotted, thick] (-1.2, 0.4) -- (-0.9, 0.15);
    \draw[fill=red] (0.4,1) circle (.05);
    \node at (0.65, 1.25) {\scriptsize $(n^b_1, n^f_1)$};
    \draw[->, densely dotted, thick] (0.45, 0.95) -- (0.45, 0.6);
    \draw[->, densely dotted, thick] (0.45, 0.95) -- (0.6925, 0.7325);
    \draw[->, densely dotted, thick] (0.45, 0.95) -- (0.8, 0.95);
  \end{tikzpicture}
  \caption{Minimizing a cost component.}
  \label{fig:vio-relu}
    \vspace{-0.8acm}
\end{wrapfigure}


